Machine Learning-Based Analysis of Sperm Videos and Participant Data for Male Fertility Prediction

Methods for automatic analysis of clinical data are usually targeted towards a specific modality and do not make use of all relevant data available. In the field of male human reproduction, clinical and biological data are not used to its fullest potential. Manual evaluation of a semen sample using a microscope is time-consuming and requires extensive training. Furthermore, the validity of manual semen analysis has been questioned due to limited reproducibility, and often high inter-personnel variation. The existing computer-aided sperm analyzer systems are not recommended for routine clinical use due to methodological challenges caused by the consistency of the semen sample. Thus, there is a need for an improved methodology. We use modern and classical machine learning techniques together with a dataset consisting of 85 videos of human semen samples and related participant data to automatically predict sperm motility. Used techniques include simple linear regression and more sophisticated methods using convolutional neural networks. Our results indicate that sperm motility prediction based on deep learning using sperm motility videos is rapid to perform and consistent. The algorithms performed worse when participant data was added. In conclusion, machine learning-based automatic analysis may become a valuable tool in male infertility investigation and research.

==> authors.tex <==

\newcommand{\oslomet}{\mbox{Blinded, Blinded}}
\newcommand{\simulamet}{\mbox{Blinded, Blined}}


\author[1,*]{Steven A. Hicks}
\author[1,+]{Vajira Thambawita}
\author[1,+]{Trine B. Haugen}
\author[1,+]{Jorunn M. Andersen}
\author[1,+]{Oliwia Witczak}
\author[1,+]{Hugo L. Hammer}
\author[1,+]{Mubarak Shah}
\author[1,+]{Michael A. Riegler}
\affil[1]{Affiliation, department, city, postcode, country}
\affil[2]{Affiliation, department, city, postcode, country}
\affil[*]{steven@simula.no}
\affil[+]{these authors contributed equally to this work}


==> tikz.tex <==


\tikzstyle{block} = [rectangle, draw, text width=5em, text centered, minimum height=4em, node distance=3cm]

\newcommand{\videoFrame}[4]{
	\def\a{#1} % Used to distinguish input resolution for current layer.
	\def\b{0.02}
	\def\c{0.1} % Width of the cube to distinguish number of input channels for current layer.
	\def\t{#2} % X offset for current layer.
	\def\d{#3} % Y offset for current layer.

	% Draw the layer body.
	\draw[line width=0.3mm](\c+\t,0,\d) -- (\c+\t,\a,\d) -- (\t,\a,\d);                                                      % back plane
	\draw[line width=0.3mm](\t,0,\a+\d) -- (\c+\t,0,\a+\d) -- (\c+\t,\a,\a+\d) -- (\t,\a,\a+\d) -- (\t,0,\a+\d); % front plane
	\draw[line width=0.3mm](\c+\t,0,\d) -- (\c+\t,0,\a+\d);
	\draw[line width=0.3mm](\c+\t,\a,\d) -- (\c+\t,\a,\a+\d);
	\draw[line width=0.3mm](\t,\a,\d) -- (\t,\a,\a+\d);

	% Recolor visible surfaces
	\filldraw[#4] (\t+\b,\b,\a+\d) -- (\c+\t-\b,\b,\a+\d) -- (\c+\t-\b,\a-\b,\a+\d) -- (\t+\b,\a-\b,\a+\d) -- (\t+\b,\b,\a+\d); % front plane
	\filldraw[#4] (\t+\b,\a,\a-\b+\d) -- (\c+\t-\b,\a,\a-\b+\d) -- (\c+\t-\b,\a,\b+\d) -- (\t+\b,\a,\b+\d);

	% Colored slice.
	\ifthenelse {\equal{#4} {}}
	{} % Do not draw colored slice if #4 is blank.
	{\filldraw[#4] (\c+\t,\b,\a-\b+\d) -- (\c+\t,\b,\b+\d) -- (\c+\t,\a-\b,\b+\d) -- (\c+\t,\a-\b,\a-\b+\d);} % Else, draw a colored slice.
}

\tikzstyle{slice} = [rectangle, draw, minimum width=1em, text centered, minimum height=4em, node distance=3cm]
\tikzstyle{line} = [draw, -latex']

==> vendor.tex <==
\begin{CCSXML}
    <ccs2012>
    <concept>
    <concept_id>10010147.10010257</concept_id>
    <concept_desc>Computing methodologies~Machine learning</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10010147.10010257.10010258.10010259.10010263</concept_id>
    <concept_desc>Computing methodologies~Supervised learning by classification</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10010147.10010178.10010224.10010225.10010230</concept_id>
    <concept_desc>Computing methodologies~Video summarization</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10010147.10010178.10010224.10010245.10010247</concept_id>
    <concept_desc>Computing methodologies~Image segmentation</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10010405.10010444.10010449</concept_id>
    <concept_desc>Applied computing~Health informatics</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Machine learning}
%\ccsdesc[500]{Computing methodologies~Supervised learning by classification}
\ccsdesc[300]{Computing methodologies~Video summarization}
%\ccsdesc[100]{Computing methodologies~Image segmentation}
\ccsdesc[500]{Applied computing~Health informatics}

\keywords{Computer assisted semen analysis, machine learning, convolutional neural networks, video analysis, regression.}

% \thanks{Contact author's address: Steven Hicks, Simula Metropolitan Center for Digital Engineering, Oslo, Norway, email: steven@simula.no}

